First Order Logic of Sparse Graphs with Given Degree Sequences

We consider limit probabilities of first order properties in random graphs with a given degree sequence. Under mild conditions on the degree sequence, we show that the closure set of limit probabilities is a finite union of closed intervals. Moreover, we characterize the degree sequences for which this closure set is the interval $[0,1]$, a property that is intimately related with the probability that the random graph is acyclic. As a side result, we compile a full description of the cycle distribution of random graphs and study their fragment (disjoint union of unicyclic components) in the subcritical regime. Finally, we amend the proof of the existence of limit probabilities for first order properties in random graphs with a given degree sequence; this result was already claimed by Lynch~[IEEE LICS 2003] but his proof contained some inaccuracies.

==> sections/fragment_size.tex <==
\subsection{Expected Size of The Fragment}





\todo[inline]{SECTION UNDER CONSTRUCTION}



Let $\Delta(n)$ be the maximum degree in $\Conf(n,\bd)$. That is
$\Delta(n)= \max \{  
d_i(n) \}$. By definition of well-behavedness, $\Delta(n)=o(n^{1/2-\epsilon})$ for some $\epsilon>0$.
Let $R=150/(\nu-1)^2$. Let $\alpha(n)= R\log(n)\Delta(n)^2$. Note that
$\alpha(n)=o(n)$. 








\begin{lemma}[Component Size in the Subcritical Phase] Assume that $\nu(\bd)<1$. For any fixed vertex $v_0\in [n]$, the probability that 
$v_0$ belongs to a component of size at least $\alpha(n)$ in $\Conf(n,\bd)$
is $o(1/n^2)$ uniformly.
\end{lemma}
\begin{proof}
The proof follows \cite{molloyCriticalPointRandom1995}[Lemma 4]. Let $V_i$ be the $i$-th exposed vertex in this exploration process. We set $V_0=v_0$. 
Let $X_0=\deg(v_0)$. For each
$i\geq 1$, let $X_i$ be the random variable counting $\deg(V_i)-2$.
\begin{claim}[1]
Suppose that $v_0$'s connected component has $T$ vertices. Then
$\sum_{i=0}^t X_i> 0$ for all 
$t < T$. 
\end{claim}
Let $Z=\sum_{i=0}^\alpha X_i$. We show that $Z$ takes negative value with high probability using Azuma's inequality
(\Cref{thm:azuma}). Suppose
$v_1,\dots, v_{i}\in [n]\setminus {v_0}$ be different vertices. 
Then
\[
\Pr(V_i=v_i \mid
V_0=v_0,\dots, V_{i-1}=v_{i-1}
)= \frac{d_{v_i}}{2m_n - \sum_{j=0}^{i-1} d_{v_j}},
\]
and
\[
\E{X_i \mid
V_0=v_0,\dots, V_{i-1}=v_{i-1}
}= 
\frac{\sum_{k=1}^n n_k k(k-2)
- \sum_{j=0}^{i-1} d_{v_j}(d_{v_j}-2)
}{2m_n - \sum_{j=0}^{i-1} d_{v_j}},
\]
It is easy to see that the expected value of $X_i$ is highest when $d_{v_j}=1$ for all $j<i$. 
\todo[inline]{Explain??}
Thus:
\[
\E{X_i \mid
V_0=v_0,\dots, V_{i-1}=v_{i-1}
}\leq 
\frac{\sum_{k=1}^n n_k k(k-2)
+ i-1 
}{m_n - i + 1} = \nu - 1 + o(1) 
\]
for all $i=i(n)\leq \alpha(n)$. Thus, for
sufficiently large $n$ the expectation above does not exceed $(\nu-1)/2$. In consequence,
$\E{Z}\leq \frac{\nu-1}{2}\alpha + d_{v_0}\leq 
\frac{\nu-1}{2}\alpha + \Delta \leq
\frac{\nu-1}{3}\alpha$ 
for $n$ sufficiently large,
independently of $v_0$.
This means that $\E{Z}$ is a growing negative value. 
Now let $v_1,\dots, v_{i-1}, v_i,
v^\prime_i \in [n]\setminus \{v_0\}
$
be different vertices, as before.
Define the events $A$ as 
$V_0=v_0,\dots, V_i=v_i$, and $A^\prime$ as
$V_0=v_0,\dots, V_{i-1}=v_{i-1},
V_i=v_i^\prime$.
We want to bound $|
\E{Z\mid A}- \E{Z\mid A^\prime}|$.
Given $j\in [n-i-2]$, we define 
$U_j$ as the $j$-th vertex in 
$[n]\setminus \{v_0,\dots, v_i, v^\prime_i\}$ 
to be exposed during the exploration process. Note that
the variables $U_j$ are independent with the events
$A$ and $A^\prime$.
Assuming the event $A$,
the set of vertices
$\{ V_{i+1},\dots, V_\alpha \}$
is formed of
$\{ U_1,\dots U_{\alpha-i-2} \}$ and an additional random vertex
$W \in [n]$.
This yields
\[
\E{Z \mid A}=
\sum_{j=0}^{i-1} \deg(v_j) 
+ \deg(v_i) + \sum_{j=0}^{\alpha-i-2}
\E{\deg(U_j)} + \deg(W).
\]
Noting that $0\leq\deg(v_j), \deg(W)
\leq \Delta$, we obtain:
\[
\sum_{j=0}^{i-1} \deg(v_j) + \sum_{j=0}^{\alpha-i-2} \E{\deg(U_j)} 
\leq \E{Z\mid A} \leq 
\sum_{j=0}^{i-1} \deg(v_j) + \sum_{j=0}^{\alpha-i-2}  \E{\deg(U_j)} + 2\Delta.
\]
By a symmetric reasoning, this inequality remains true
for $\E{Z\mid A^\prime}$. From this
we obtain $\left|\E{Z\mid A} - \E{Z\mid A^\prime}\right|\leq 2\Delta$. \par
By Azuma's inequality,
\[
\Pr(| Z - \E{Z}| \geq \epsilon)\leq 
2\exp\left(\frac{-\epsilon^2}{8\alpha \Delta^2}
\right).
\]
In particular, as $\E{Z}\leq  \frac{\nu-1}{3} \alpha < 0$, 
\[
\Pr( Z \geq 0)\leq 
2\exp\left(\frac{-(\nu-1)^2 \alpha^2}{72\ \alpha \Delta^2}
\right)=2\exp\left(\frac{ 150\ log(n)}{72}
\right)=o(n^{-2}).
\]
Note that this bound holds uniformly for all choices of $v_0$.
The fact that $Z<0$ implies
$v_0$'s connected component has
less than $\alpha$ vertices, so last
inequality proves the result. 
\end{proof}



\begin{corollary}
\label{}
\label{ch:degs.cor:cmp_expected_size}
Assume $\nu<1$.
Given a vertex $v\in [n]$, let $Z_n(v)$
be the random variable measuring the size
of $v$'s connected component in $\Conf(n,\bd)$.
Then
\[
\max_{v\in [n]} \left(\frac{\nu}{1-\nu} - \frac{\E{Z_n(v)}}{d_v(n)} \right)
= o\left(
1\right).
\]
\end{corollary}
\begin{proof}
	Let $\alpha(n)=R \log(n) \Delta(n)^2$ be as in the previous theorem. Consider
	the biased
	degree distribution 
	$\HD^\prime(n)$
	obtained by removing $\alpha(n)$ degree-one vertices from $\Conf(n,\bd)$. That is, 
	\[
	\Pr(\HD^\prime(n)=i-1) = 
	\begin{cases}
		\dfrac{n_i i }{2m_n -\alpha(n)} \text{ if $i>1$, and }\\ 
		\dfrac{n_i - \alpha(n)}{2m_n -\alpha(n)} \text{ otherwise.}
	\end{cases}
	\]
    As $\alpha(n)=o(n)$, the following hold: 
	(1) $\E{\HD^\prime(n)}=\nu +  o(1)$, and (2) $\HD^\prime(n)$ stochastically dominates $\HD(n)$.
	
	Let $v_0\in [n]$ be an arbitrary vertex. Consider the exploration process defined in REF. Let $V_i$ be the $i$-th exposed vertex during this process, and let $X_i=\deg(V_i)-1$ for $i>0$, $X_0=\deg(v_0)+1$, as before. 
	Note that
	$X_i$ is stochastically dominated by $\HD^\prime(n)$ for all $1\leq i\leq \alpha$.
	Let $Y$ be the indicator variable
	$\one_{
	\{Z_n(v_0)\leq \alpha\}}$.
	For each $i$ we define the random variable
	$\bar{X}_i= X_i Y$.
	Consider a branching process $BP$
	with offspring distribution $\HD^\prime(n)$, offspring variables $X^\prime_i$, and root degree $X_0=\deg(v_0)$.
	Let $T$ be the smallest number such that $\sum_{i=0}^T \bar{X}_i=T$
	let $T^\prime$ 
	be the total progeny of 
	$BP$. It holds that
    $Z_n(v_0)Y \leq T$, and $\E{T}\leq \E{T^\prime}$. Thus,
    $\E{ Z_n(v_0)Y}\leq \E{T^\prime}$.
    Now we bound $\E{Z_n(v_0)}$.
    \[
    \E{Z_n(v_0)}=
    \E{Z_n(v_0)Y} + \E{Z_n(v_0)(1-Y)}
    \leq \E{T^\prime} + n\E{1-Y}.\]
    We bound the last two terms now. 
    Consider $\E{T^\prime}$ first. 
    By REF, this expected total progeny equals $d_{v_0}\E{D^\prime(n)}/
    (1-\E{D^\prime(n)}$, which is
    $d_{v_0}\left(\frac{\nu}{1-\nu} + o(1) \right)$. Now let us take a look at $n\E{1-Y}$. By last theorem $\E{1-Y}=o(n^2)$. Putting everything together we obtain
    \[
    \E{Z_n(v_0)}\leq
    d_{v_0}\left(\frac{\nu}{1-\nu} + o(1) \right) + o(1/n),
    \]
    which proves the result. 
 
\end{proof}



\begin{theorem}
Assume that $\nu<1$.
Let $A_{n,k}$ be the event that
$\Conf(n,\bd)$ contains a unicyclic component of size $k$.
For any $\epsilon>0$ there is a bound $K_\epsilon$ such that
\[\lim_{n\to \infty}\Pr( A_{n,K_\epsilon})< \epsilon.\]
\end{theorem}

The proof follows from three facts. First, with high probability $\Conf(n,\bd)$ contains no 'large' cycles. Second, w.h.p. small cycles in
$\Conf(n,\bd)$ contain no 'large' degree vertex. Finally, given a small cycle formed of small-degree vertices, w.h.p. the connected region 'growing out' of each vertex is small. These three facts together imply that w.h.p. no large unicyclic components occur in $\Conf(n,\bd)$. \par
\begin{claim}[1]
Let $P^{(1)}_\ell(n)$ be the event that $\Conf(n,\bd)$ contains some cycle of length
greater than $\ell$. Then there exists some $L$
satisfying $\Pr(P^{(1)}_L(n))<\epsilon/3$
for sufficiently large $n$.
\end{claim}
\begin{proof}
Let $Z_i(n)$ be the number of $i$-cycles in
$\Conf(n,\bd)$.
By \Cref{lem:cycle_count_conf}, 
$(\E{Z_i(n)})_{i\geq 1}$ is uniformly summable. Thus, there is some $L$ such that 
$\lim_{n\to \infty} \sum_{i> L} \E{Z_i(n)} < \epsilon/3$. By Markov's inequality this implies that $\Conf(n,\bd)$ has no $i$-cycles
for $i>L$ with probability $1-\epsilon/3$, as $n$ tends to infinity. 
\end{proof}
\begin{claim}
Fix $L\geq 1$.
Let $P^{(2)}_{L,a}(n)$ be the event that
some cycle of length
at most $L$ lying in $\Conf(n,\bd)$
contains a vertex $v\in [n]$ of degree
greater than $a$. Then there exists some $a$
satisfying $\Pr(P^{(2)}_{L,a}(n))<\epsilon/3$
for sufficiently large $n$.
\end{claim}
\begin{proof}
Let $Z_{l,a}(n)$ be the number of $l$-cycles
in $\Conf(n,\bd)$ containing some vertex
$v$ with $d_v(n)>a$. Note that
$Z_{l,a}(n)< Z_{l}(n)$, so
by \Cref{lem:cycle_count_conf}
the sequence
$(\E{Z_{l,a}(n)})_{l\geq 1}$ is uniformly summable for all $a$.
Let $\Hinge_l(n)$ be the set of hinge-sequences defined in \Cref{lem:cycle_count_conf}. Among these,
let $\Hinge_{l,a}(n)\subseteq \Hinge_l(n)$
contain the hinge-sequences $(e_1,h_1),\dots,(e_l,h_l)$, where $(e_1, 
h_1)$ belongs to a vertex with degree greater than $a$. It holds that
\[
\E{Z_{\ell,a}(n)}\leq
\frac{\Hinge_{\ell,a}(n)}{(m_n - 1) (m_n -3) 
\cdots (m_n - 2\ell +1)}.
\]
Let $Q_a(n)=\sum_{i>a} n_i i (i-1)$.
The fact that $n_i/n i(i-1)$
converges to $\lambda_i i(i-1)$ uniformly
implies that for sufficiently large $a$
$Q_a(n)< n\epsilon\rho_1\frac{1}{6L}$ for all $n$.
As before, we can deduce the bound $|\Hinge_{\ell,a}(n)|\leq
Q_a(n)
(\Hinge(n)-2)
(\Hinge(n)-4)\cdots (\Hinge(n) - 2\ell)
$. Thus,
\[
\E{Z_{\ell,a}(n)}\leq
\frac{Q_a(n)}{m_n-1}\left(
\frac{\Hinge(n)}{(m_n - 1)}\right)^{\ell-1}
= \frac{\epsilon}{6L}\nu^\ell + o(1)
\leq \frac{\epsilon}{6L}+ o(1)
\]
This implies
$
\sum_{\ell=1}^L 
\E{Z_{\ell,a}(n)} \leq \frac{\epsilon}{6} + o(1)$, and by Markov's inequality 
$\Pr(\sum_{\ell=1}^L Z_{\ell,a}\geq 1) < \epsilon/3$ for sufficiently large $n$. 
\end{proof}
\begin{claim}
Fix $L,a\geq 1$. Let $P^{(3)}_{L,a,k}(n)$ be the event that $\Conf(n,\bd)$ 
has a unicyclic component $C$ of size $n_C> k$ containing a cycle of length at most $L$ whose vertices have
all degree at most $a$. Then there exists
some $K$ satisfying
$\Pr(P^{(3)}_{L,a,K}(n))<\epsilon/3$ for sufficiently large $n$.
\end{claim}
\begin{proof}


\end{proof}

Given a set of
half-edges $S\subseteq [2m_n]$,
we define the multigraph 
$\Conf(n,\bd)\setminus S$ 
as the one obtained from $\Conf(n,\bd)$
by removing all edges containing some half-edge
in $S$. \par
Let $\Pi_{L,a}\subseteq \NN^*$ be the set of sequences
$\bm{x}=(x_1,\dots, x_\ell)$ where
$\ell\leq L$ and $2\leq x_i \leq a$ 
and $\lambda_{x_i}\neq 0$ for all $i$. Additionally, for such $\bm{x}$, we define
$[n]_{\bm{x}}$ as the set of tuples
$(v_1,\dots,v_\ell)$ where $d_{v_i}(n)=x_i$
for all $i$.
Let $Z_{L,a}(n)$ be the random variable counting the vertices belonging to unicyclic components of $\Conf(n,\bd)$ where the cycle has length at most $L$ and is formed of vertices with degree at most $a$. It holds:
\[
\E{Z_{L,a}(n)}= 
\sum_{
\bm{x} \in \Pi_{L,a}, \,
\bm{v}\in [n]_{\bm{x}}
}
\frac{1}{2|\bm{x}|}
\Pr(\bm{v} \text{ forms a cycle})\cdot
\E{ C_{\bm{v}}(n) \mid \bm{ v } \text{ forms a cycle}}.
\]

Note that the term inside has the same value for all tuples of vertices $\bm{v}$
corresponding to the same sequence of degrees 
$\bm{x}\in \Gamma_{L,a}$. 
Thus, it makes sense to fix a sequence of vertices $\bm{v}^{(\bm{x},n)}  \in [n]_{\bm{x}}$ for all $\bm{x}\in \Gamma_{L,a}$
and sufficiently large $n$. Additionally, for
each $n$ fix a partial matching $M_{\bm{x}}(n) \subseteq \binom{[2m_n]}{2}$ realizing a cycle
formed by the vertices
$\bm{v}^{(\bm{x},n)}$ in the
given order. This way, we can rewrite last equation as
\[
\E{Z_{L,a}(n)}= 
\sum_{
\bm{x}\in \Pi_{L,a}
}
\frac{\left|[n]_{\bm{x}}\right|}{2|\bm{x}|}
\Pr(\bm{v}^{(\bm{x},n)}  \text{ forms a cycle})\cdot
\E{ C_{\bm{v}^{(\bm{x},n)} }(n) \mid 
M_{\bm{x}}(n)}.
\]
There is a finite number of
degree-tuples in $\Pi_{L,a}$. Hence, to show
$\E{Z_{L,a}(n)}$ is bounded,
it suffices to show this for each of the terms in the r.h.s. sum.
Let us examine those terms in greater detail.
Fix a degree-tuple $\bm{x}\in \Pi_{L,a}$,
let $\bm{v}^{(n)}=\bm{v}^{(\bm{x},n)}$
and $M(n)=M_{\bm{x}}(n)$.
The
probability that $\bm{v}^{n}$ forms a cycle is exactly
$
\prod_{i=1}^{|\bm{x}|}
\frac{ x_i(x_i-1)}{
(2m_n -2i + 1)}
$. Additionally, $|[n]_{\bm{x}}|$ is at most
$\prod_{i=1}^{|\bm{x}|} n_{x_i}$. This yields
\[
\big|[n]_{\bm{x}}\big| \cdot
\Pr(\bm{v}^{(n)}  \text{ forms a cycle})
\leq
\prod_{i=1}^{|\bm{x}|}
\frac{ n_{x_i} x_i(x_i-1)}{
(2m_n -2i + 1)}= \prod_{i=1}^{|\bm{x}|} 
\frac{\lambda_{x_i}x_i(x_i-1)}{\mmnt_1} + o(1).
\]
This expression is clearly bounded,
implying that
$\E{Z_{L,a}(n)}$ is bounded iff \linebreak
$\E{ \lvert \Cmp(\bm{v}^{(n)},n) \lvert \mmid M(n)}$ is so. Let $\widehat{\Cmp}(v_i^{(n)},n)$ be the connected component of $v^{(n)}_i$ in 
$\Conf(\bd,n)\setminus M(n)$, for 
each $1\leq i \leq |\bm{x}|$. 
Assuming that
the matching $M_(n)$ occurs in
$\Conf(n,\bd)$, it follows
$\Cmp(\bm{v}^{(\bm{x},n)},n)$ contains the cycle realized
by the matching $M(n)$, and all the vertices
$u$ connected to this cycle.
Each one of these vertices $u$ has a path to some $v^{(n)}_i$ that does not use any half edge in $M(n)$. 
This way, $\left(
\Cmp(\bm{v}^{(n)},n) 
\mmid M(n) \right) =$
$
\cup_{i=1}^{|\bm{x}|}
\widehat{\Cmp}(v_i^{(n)},n)$.
This implies
\[
\E{|\Cmp(\bm{v}^{(n)},n)| \mmid
M(n)} \leq
\sum_{i=1}^{|\bm{x}|}
\E{
\lvert\widehat{\Cmp}(v^{(n)}_i,n)\rvert
}.
\]
Define the modified degree sequence
$\widehat{\bd}(n)$ by setting 
$\widehat{d}_v(n)=d_v(n)- 2$ if $v=v^{(n)}_i$
for some $1\leq 1 \leq |\bm{x}|$, and
$\widehat{d}_v(n)= d_v(n)$ otherwise. Intuitively, $\widehat{d}(n)$ is the degree sequence obtained from $\bd(n)$ after removing the half-edges in the cycle $M(n)$. 
Note that the moments of the degree distribution given by $\widehat{\bd}(n)$
converge to those of $\bd(n)$. Additionally,
$\Conf(n,\bd)\setminus M(n) \sim
\Conf(n,\widehat{\bd})$. Thus, from \Cref{ch:degs.cor:cmp_expected_size} 
follows that $\E{
\lvert\widehat{\Cmp}(v^{(n)}_i,n)\rvert
}= x_i \frac{\nu}{1-\nu}+ o(1)$.
This proves
$\E{Z_{L,a}(n)}$ is bounded.


==> sections/local_convergence.tex <==

\label{sec:local}

\begin{definition}[Breadth-First Exploration From a Set of Roots]
\label{def:exploration}
Let $v_1,\dots, v_k$ be a sequence of different vertices in $[n]$, called \textbf{roots}. The following exploration process exposes
the connected components of the roots in 
$\Conf(n,\bd)$ following a breadth-first order.
This way, the process returns a partial matching $M\subseteq \binom{[2m_n]}{2}$ corresponding to those connected components.
During the procedure, 
we partition the set $[2m_n]$ of half-edges
into three sets $A, I, D$. Half-edges in $A$, $B$,
and $C$ are called \textbf{active}, \textbf{inactive}, and \textbf{dead}, respectively.
The set $A$ of active half-edges is an ordered list. A vertex $v\in [n]$ is called \textbf{unexposed} if all its half-edges are inactive, \textbf{partially exposed}
if it has some active half-edge, and \textbf{fully exposed} if all its half-edges are dead. 
We adopt the convention that non-root degree-zero vertices are unexposed, and degree-zero roots are fully exposed. 
The process occurs in two steps:
\begin{itemize}
    \item[1.] Initialize $A$ as 
    $v_1$'s half-edges (in order), followed by 
    $v_2$'s half-edges, and so on, finishing with
    $v_k$'s half edges. Mark the half-edges in $A$
    as active. Set $D=\emptyset$, $I=[2m_n]\setminus A$.
    \item[2.] Repeat until $A$ is empty: Move 
    the first half-edge $e$ in $A$ to $D$. Choose a remaining alive half-edge 
    $h\in I\cup A$ uniformly at random and move it to $D$ as well. Add the pair $(e,h)$ to $M$.
    If $h$
    was inactive and belongs to a vertex $u$, 
    move the rest of $u$'s half-edges to the end of $A$ maintaining their order. 
\end{itemize}
\end{definition}

A \textbf{rooted} multi-graph
$(G,\bm{v})$
is simply a multi-graph $G$ equipped with a tuple of distinguished vertices
$\bm{v}\in (V(G))^*$, called roots.
Note that the roots are given by an ordered tuple.
Two rooted multi-graphs
$(G_1,\bm{v}^{1}), ( G_2, \bm{v}^{2})$
are isomorphic if there is an isomorphism between the underlying multi-graphs $G_1,G_2$ which maps
$\bm{v}^{1}$ to $\bm{v}^2$. An \textbf{unlabeled rooted multi-graph}
is an isomorphism class of rooted multi-graphs. \par
Let $G$ be a multigraph, and let 
$\bm{v}\in (V(G))^*$ be a tuple
of roots. The
$r$-\textbf{neighborhood} of $\bm{v}$, denoted $N_G(\bm{v},r)$, is the rooted multi-graph $(H,\bm{v})$, where $H$
is the multi-graph induced by $G$
on the vertices 
\[
V(H)= \{ u\in V(G) \mid d_G(u,v_i)\leq  r \text{ for some } v_i \}.
\]

Let $N_n(\bm{v},r)= N_{\Conf(n,\bd)}(\bm{v}, r)$. 

\begin{theorem} 
Fix $k\geq 1$.
For each $n$, let
$V_1(n),\dots, V_k(n)$
be i.i.d. uniformly random vertices in $[n]$. Let $\BP$ be a $k$-root branching process with root offspring distribution $D$, and general 
offspring distribution $\widehat{D}$.
Let $\Tcal$ be a rooted forest
with $k$ roots and height at most $r$. Then
\[
\Pr(N_n(\bm{v},r)\simeq \Tcal)
=\Pr(\BP\vert_r \simeq \Tcal)+ o(1).
\]
\end{theorem}
\begin{proof}
Consider the  
exploration process $\mathrm{G}$ defined in \Cref{def:exploration},
starting from the roots $V_1(n),\dots, V_k(n)$. We describe a coupling with a $k$-root branching process $\BP(n)$ with root offspring distribution $D(n)$ and general offspring distribution $\widehat{D}(n)$. \par
Let $(E_j)_{j\geq 1}$ denote the alive half-edge $h$ chosen during the $j$-th
iteration of Step 2 in $\mathrm{G}$.
Let $(X_i)_{i\geq 1}$ be the offspring variables of $\BP(n)$.
We consider a sequence $(E^\prime_j)_{j\geq 1}$ of i.i.d. random half edges in $[2m_n]$, chosen uniformly at random. We couple $\BP$ and $\mathrm{G}$ as follows: 
We begin by defining $\BP$. For
$1\leq i \leq k$ we set 
$X_i=d_{V_i}(n)$. For $i> k$ 
$X_i$ is defined as $d_{U_{i-k}}(n) - 1$,
where $U_{i-k}$ is the vertex corresponding to the random half-edge 
$E^\prime_{i-k}$.
Now we define $\mathrm{G}$. For each
$j\geq 1$ we define $E_j=E^\prime_j$
if the half-edge $E^\prime_j$ is still alive in the exploration. Otherwise, if $E^\prime_j$ is already dead, then 
we say the coupling \textbf{failed} 
and $(E_\ell)_{\ell\geq j}$ continue independently of $(E^\prime_\ell)_{\ell\geq j}$.
If $\mathcal{G}_t\not\simeq \BP_t$ then one of the following holds: 
\begin{enumerate}[label=(\Roman*)]
    \item The coupling between $E_j$
    and $E^\prime_j$ has failed for $j\leq t$.
    \item Some half-edge
    $E^\prime_j$ with $1\leq j\leq t$
    belongs to one of the vertices
    $V_1,\dots, V_k$.
    \item Some half-edges
    $E^\prime_i, E^\prime_j$ with
    $1\leq i < j \leq t$ belong to the same vertex. 
\end{enumerate}
We show that the probability of either these events occurring is $o(1)$.
The probability that (I) holds for a fixed $j$ is precisely $\frac{2(j-1)}{2m_n}$, as there are 
$2(j-1)$ dead half-edges when the 
$j$-th round of $\mathrm{G}$ starts.
Thus, using the union bound, the probability that (I) holds is at most
$\sum_{j=1}^t \frac{2(j-1)}{2m_n}= o(1)$.
The probability that (II) holds for a fixed $j$ is exactly 
$\frac{\sum_{i\in [k]} 
d_{V_i}}{2m_n}$, which is at most
$\frac{k\Delta}{2m_n}$. Using the union bound as before, we get that
(II) occurs with at most 
$\frac{t k\Delta}{2m_n}=o(1)$ probability. Finally the probability that (III) holds for a choice of $i<j$, is $\frac{(d_{U_i}-1)}{m_n}$,
where $U_i$ is the vertex corresponding to the random half-edge $E^\prime_i$. Summing over all pairs,
the probability that (III) happens is at most $\frac{t^2\Delta}{m_n}=o(1)$.
This shows that $\DTV(\mathrm{G}_t(n),
\BP_t(n))=o(1)$
over unlabeled rooted multi-graphs. As $\BP_t(n)$ converges in distribution to $\BP_t$, so does $\mathrm{G}_t(n)$.
Now the result follows taking into account that $\BP\vert_r\simeq \Tcal$ iff $\BP_t \simeq \Tcal$, where 
$t$ is the number of non-root vertices in the first $r-1$ generations of $\Tcal$.
\end{proof}


\begin{definition}

We call a $r$-\textbf{fragment} to a fragment where all cycles have length at most $2r+1$ and all vertices belong to the $r$-neighborhood of a cycle.   
Let $G$ be a multigraph, and let $\ell, r\in \NN$. Let $U \subseteq V(G)$ be the vertices
belonging to some cycle in $G$ which has length at most $\ell$. Let $H \subseteq G$ be the
sub-graph induced by $G$ on all its vertices whose distance to $U$ is at most $r$.
The $r$-\textbf{fragment} of $G$, written $\Frag_G(r)$, is the fragment $\Frag_H$. We write $\Frag^*_n(r)$ for $\Frag_{\Conf(n,\bd)}(r)$.
\end{definition}




\begin{lemma}
\label{lem:r_frag}
Let $r>0$. 
Let $H$ be a $r$-fragment.
Let $h$ be the number of vertices in $H$ which have height at most $r-1$, and let $h_i$
be the number of those who have degree $i$. Then
\[
\Pr(\Frag^*_n(r)\simeq H)
=  \frac{e^{-\sum_{s=1}^{2r+1} \nu^s/2s}}{\aut(H)\mmnt_1^{h}} 
\prod_{i\geq 1}\left( \lambda_i i!\right)^{h_i}.
\]
\end{lemma}
\begin{proof}
Let $S\subseteq V(H)$ be the set of vertices in $H$ whose height is at most $r-1$, and let $S^\prime$ be the set of those with height exactly  $r-1$. Define $\Fcal(n)$ as the set of injective maps $f:S\rightarrow [n]$ that are degree-preserving.
For each $f\in \Fcal(n)$, let $A_f$ be the event that $f$ is a partial isomorphism that can be extended into an isomorphism between $H$ and
$\Frag^*_n(r)$. Then
$\Pr(\Frag^*_n(r)\simeq H)
= \sum_{f\in \Fcal(n)} \Pr(A_f)$.
By symmetry, $\Pr(A_f)$ is the same for all $f\in \Fcal(n)$. It is also easy to see that for any $f,g\in \Fcal(n)$, the events $A_f, A_g$ can either coincide or be disjoint. 
Let $\Phi_H$ be the set of maps $\phi: S\rightarrow S$ that can be extended into automorphisms of $H$. 
Then $A_f$ and $A_g$ coincide iff $f=g\circ \phi$ for some $\phi\in\Phi_H$. Otherwise $A_f$ and $A_g$ are disjoint. 
Fix a choice $f_n\in \Fcal(n)$ for each $n$. Then 
\begin{equation}
\label{lem:r_frag.eqn:1}
 \Pr(\Frag^*_n(r)\simeq H)
= \frac{|\Fcal(n)|}{|\Phi_H|} \Pr(A_{f_n}).
\end{equation}
Observe that $|\Fcal(n)|$ is precisely 
$\prod_{i\geq 1} (n_i)_{h_i}$. Let us examine now $|\Phi_H|$. Let $\phi \in \Phi_H$. Then $\phi$ can be extended into an automorphism of $H$ in exactly  $\prod_{v\in S^\prime} (\deg(v)-1)!$ different ways. Indeed, these extensions are given by different orderings of the ``leaves'' attached to each
$(r-1)$-height vertex in $H$. This way, 
$
|\Phi_H|= \aut(H) \big/ \prod_{v\in S^\prime}
(\deg(v)-1)!
$. Plugging our newly obtained expressions for 
$|\Fcal(n)|$ and $|\Phi_H|$ into \cref{lem:r_frag.eqn:1} we get
\begin{equation}
\label{lem:r_frag.eqn:2}
 \Pr(\Frag^*_n(r)\simeq H)
= \frac{\Big(\prod_{i\geq 1} (n_i)_{h_i}\Big) \Big( \prod_{v\in S^\prime}(\deg(v)-1)! \Big)}{\aut(H)} \Pr(A_{f_n}).
\end{equation}
We turn now to computing $\Pr(A_{f_n})$. Let
$P_n$ be the event that $\Conf(n,\bd)$ is $r$-simple. By REF, $\Pr(A_{f_n})=\Pr(A_{f_n}\wedge P_n) + o(1)$.
We focus on the probability $\Pr(A_{f_n}\wedge P_n)$. Define $\widehat{G}_n$ as the multigraph that results from deleting all edges between vertices in $f_n(S)$ from $\Conf(n, \bd)$. 
Let us define the following events:
\begin{itemize}
    \item $\mathrm{Hom}_n$: $f_n$ is an homomorphism
    \item $\mathrm{Cycles}_n$: All cycles in $\widehat{G}_n$ have length bigger than $2r+1$. 
    \item $\mathrm{Paths}_n$: 
    In $\widehat{G}_n$, all vertices
    $v_1,v_2\in f(S^\prime)$ lie at distance bigger than $2r+1$ from each other.  
\end{itemize}
By definition 
$A_{f_n}\wedge P_n$ is equivalent to 
$\mathrm{Hom}_n\wedge \mathrm{Cycles}_n
\wedge \mathrm{Paths}_n$. The probability of 
$\mathrm{Hom}_n$ is exactly
$Pr($



\end{proof}

